Neutron detector response modeling in NOvA

Neutrons can present a significant challenge for neutrino experiments in which energy reconstruction is critical. With the ability to escape detection completely and with a weak correlation between their kinetic energy and any eventual energy deposition, it is difficult to fully account for neutrons produced in neutrino interactions. This in turn leads to significant model dependence when evaluating neutron-related systematic uncertainties. The NOvA experiment is a long-baseline neutrino oscillation experiment with a high-statistics sample of antineutrino data collected by its near detector. We report an excess relative to data of simulated neutron candidates with low energy depositions when using standard Geant4 physics lists. The simulation excess is traced to an overabundance of secondary photons produced from interactions of neutrons with kinetic energy greater than \SI{20}{\mega\eV}. Improved agreement with data is obtained by applying the data-driven neutron-on-carbon \menate model for neutrons between \SI{20}{\mega\eV} and ${\sim}$\SI{100}{\mega\eV}. With \menate, the residual oversimulation is more uniform across the calorimetric neutron energy spectrum, suggesting possible overproduction of primary neutrons by the GENIE neutrino interaction generator. These results motivate the adoption of \menate-supplemented Geant4 simulation as the nominal simulation in the production of future \nova simulation.

==> preamble.tex <==
\usepackage{graphicx}
\usepackage{xspace}
\usepackage{siunitx}
\sisetup{range-phrase=--}
\sisetup{range-units=single}
\usepackage{multicol}
\usepackage{amsmath}
\makeatletter
\providecommand*\caption@documentclass{standard}
\makeatother
\usepackage{subcaption}
\usepackage{cleveref}
\newcommand{\crefrangeconjunction}{--}


% This prevents line numbers for the right column from nearly overlapping the text
% in the left column.

\usepackage{xurl}

%
% Keeps figures with sections
%\usepackage[section]{placeins}
%\makeatletter
%\AtBeginDocument{%
%  \expandafter\renewcommand\expandafter\subsection\expandafter{%
%    \expandafter\@fb@secFB\subsection
%  }%
%}
%\makeatother


% \oset macro for nice over-bar parentheses:
\makeatletter
\newcommand{\oset}[3][0ex]{%
  \mathrel{\mathop{#3}\limits^{
    \vbox to#1{\kern-2.5\ex@
    \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother

\newcommand\barbracket[1]{\oset{%
   \scriptscriptstyle(\textbf{--})}{#1}}

\newcommand\overbar[1]{\oset[-0.5ex]{%
   \textbf{--}}{#1}}   

%New Commands (can probably cut these down a lot}
\newcommand{\nueParen}{\ensuremath{{\nu}_{e}~(\bar{\nu}_{e})}\xspace}
\newcommand{\numubar}{\ensuremath{\overbar{\nu}_\mu}\xspace}
\newcommand{\numuParen}{\ensuremath{{\nu}_{\mu}~(\bar{\nu}_{\mu})}\xspace}

\newcommand{\numutonueParen}{\numuParen{}\,$\rightarrow$\,\nueParen}
\newcommand{\numutonumuParen}{\numuParen{}\,$\rightarrow$\,\numuParen}


\newcommand{\nova}{NOvA\xspace}
\newcommand{\menate}{MENATE\xspace}
\newcommand{\menater}{MENATE\_R\xspace}




